Enabling Tensor Decomposition for Time-Series Classification via A Simple Pseudo-Laplacian Contrast

Tensor decomposition has emerged as a prominent technique to learn low-dimensional representation under the supervision of reconstruction error, primarily benefiting data inference tasks like completion and imputation, but not classification task. We argue that the non-uniqueness and rotation invariance of tensor decomposition allow us to identify the directions with largest class-variability and simple graph Laplacian can effectively achieve this objective. Therefore we propose a novel Pseudo Laplacian Contrast (PLC) tensor decomposition framework, which integrates the data augmentation and cross-view Laplacian to enable the extraction of class-aware representations while effectively capturing the intrinsic low-rank structure within reconstruction constraint. An unsupervised alternative optimization algorithm is further developed to iteratively estimate the pseudo graph and minimize the loss using Alternating Least Square (ALS). Extensive experimental results on various datasets demonstrate the effectiveness of our approach.

==> sections/introduction.tex <==
\section{Introduction}

\re{

\textbf{Tensor decomposition is known for its suboptimal performance in classification tasks} \cite{}:  Tensor decomposition, originally as a dimension-reduction method, although has been successfully applied to multi-dimensional time-series data, such as in neuroscience \cite{cong2015tensor}, transportation \cite{chen2019bayesian} and economics \cite{wang2022high}, however, it is mainly fitted for regression-like tasks: prediction \cite{li2020tensor,li2020long} and imputation \cite{chen2019bayesian}. The reason is stemmed from the way how the decomposition is learned: take the CANDECOMP/PARAFAC (CP) tensor decomposition \cite{k:09} on a three-dimensional tensor $\mathcal{X}$ as an example, $\mathcal{X}$ is decomposed into three mode matrices along each dimension, $\mathbf{A,B,C}$, with a weight vector $\mathbf{w}$; however, \re{as shown in Fig. \ref{fig:motivation}} (a), $\mathbf{w,A,B,C}$ are only learned by minimizing the \textit{reconstruction loss} $\| \mathcal{X} - \llbracket  \mathbf{w,A,B,C} \rrbracket \|_2^2$ (with details later). This creates two problems of the decomposition results: nonuniqueness \cite{k:09} and rotation invariance \cite{k:09}, e.g., the decomposed $\mathbf{w}$ can be scaled, transformed, or rotated in each decomposition, even under the same reconstruction loss. This won't be a problem for regression-like tasks, but it will significantly affect the classification task since most of the tensor-based classification paradigms uses the decomposed $\mathbf{w}$ as the feature vector of each sample. As a result, shown in Fig. \ref{fig:motivation}(a), the features are learned with all class patterns messily mixed.

ATD \cite{y:22}, is the first attempt to not only respect the \textit{fitness} of tensor decomposition (to minimize reconstruction loss), but also the \textit{alignment}. It proposed an instance-wise \textit{contrastive loss} for alignment, where only $\mathbf{w}$ and its direct augmented sample $\widetilde{\mathbf{w}}$ are positive sample: this is reasonable since class labels are unknown when training the tensor decomposition, then only a sample and its augmented one can be 100\% guaranteed as positive. However, such an instance-wise alignment may even harm the pattern learning: (1) as shown in Fig \ref{fig:motivation}(b), it will treat other samples from the same class as negative samples, which harms the performance (\textbf{-\#\%} worse than ours); \re{(2) we prove that such a instance-contrast loss is a lower bounded by ours, showing that its intra-class is less compact and inter-class is less separate as ours, as we can see by comparing Fig. \ref{fig:motivation}(c) with (b)} \man{ %(2) its class-aware distinctiveness in the feature space will be obscured without considering both the inter- and intra-class distances;
(3) ignoring of the diversity of samples within the same class may lead to over-fitting issue, thereby reducing generalizability.}\re{e.g., due to a limited knowledge of a class, it needs more \textbf{$\times$\# times} more samples for supervised training of the classifier to achieve similar result as ours}
%\ziyue{being prone to overfitting and lacking generalizability? since the positive samples ignore the diversity of samples from a same class}; (3) anymore? (same as the disadvantage of instance SSL vs block ssl)

}

\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{figure/motivation3.pdf}
\caption{ The class information in the feature space: (a) the features extracted by CP decomposition are messed together; (b) instance-wise contrast (e.g., ATD \cite{y:22} and InfoNCE \cite{oord2018representation}) treating the data from the same instances as a positive pair only presents obscure class patterns; (c) block-wise contrast (e.g., PCL \cite{li2020prototypical} and CURL \cite{arora2019theoretical}) guided by pseudo graph is more class-distinctive. ( $\dashleftarrow\dashrightarrow$: pull far away, $\rightarrow\leftarrow$: push closer with darker color indicating more impact). \ziyue{(1) no need to draw the different class's negative samples, maybe only highlight the purple class?; (2) highlight the label is unknown, so we need to learn a pseudo graph to have the light-orange links; (3) add fig (d): the pseudo graph and feature are cyclically improving each other}}
\label{fig:motivation}
% \vspace{-0.3cm}
\end{figure*}

% \re{nonuniqueness and rotation invariance (toy experiment: repeat the CP decomposition for N times and plot their t-sne to see whether some have better class information) -> class-alignment}

\re{To address the weakness of instance-wise contrastive learning, our solution comes intuitively yet effectively: \textbf{can we construct a pseudo graph indicating which samples are from the same class based on learned features, and then use the graph to improve the feature in return}?} Specifically, \re{apart from the reconstruction loss}, such a pseudo graph is introduced as auxiliary information to guide the graph contrast, and augmentation-based instance contrast is also included to mitigate class-irrelevant noise. Then we jointly optimize the contrastive objectives and tensor decomposition reconstruction objective using Alternative Least Square (ALS).

\re{

As a result, via such an iterative updating between pseudo graph and feature, similar to EM algorithm:

(1) not only our features are improved to preserve more class pattern (with \textbf{+\#\%} higher classification accuracy and clearer separation in the embedding space in Fig. \#), (2) the learned pseudo graph is also close to the ground truth (in Figure \#). This is also proved by the small margin of \#\% comparing with using the ground truth label for guidance, instead of pseudo graph. (3) We show that the pseudo graph contrast is similar to the classical SampledNCE framework \cite{hamilton2017inductive}, but with a well-designed Laplacian matrix that gives a different impact of different contrast sources and also enjoys the block-wise contrastive property of being more compact and preserving more class information. (4) We also show a great insight that the tensor decomposition is a two-edge sword as shown in Fig. \ref{fig:overview}(b) ; as mentioned before, the decomposition result is not identifiable and rotation-invariant: firstly, due to the non-uniqueness, the reconstruction loss provides a bunch of nonidentifiable decomposition results with a small $\epsilon$ region; then, thanks to the rotation-invariance, our pseudo graph contrast is actually ``rotating'' the decomposition result to an angel that maps the class pattern to the most while maintaining the same reconstruction loss. 

}

\begin{comment}
\man{
    As a result, via such an iterative updating between pseudo graph and feature, similar to EM algorithm, we can achieve:
    \begin{itemize}
        \item Better intrinsic class-aware representation learning: not only our features are improved to preserve more class pattern (with \textbf{+\#\%} higher classification accuracy and clearer separation in the embedding space in Fig. \#), (2) the learned pseudo graph is also close to the ground truth (in Figure \#). This is also proved by the small margin of \#\% comparing with using the ground truth label for guidance, instead of pseudo graph. 
        \item Better generalization for small labeled dataset: We show that the pseudo graph contrast is similar to the classical SampledNCE framework \cite{hamilton2017inductive}, but with a well-designed Laplacian matrix that gives a different impact of different contrast sources and also enjoys the block-wise contrastive property that the feature space itself is more class distinctive.
        \item Great insights that the tensor decomposition is a two-edge sword: as mentioned before, the decomposition result is not identifiable and rotation-invariant: firstly, the reconstruction loss guarantees the decomposition results stay within a small $\epsilon$ region; then, our pseudo graph contrast is actually ``rotating'' the decomposition result to an angel that maps the class pattern to the most. 
    \end{itemize}
}
\end{comment}
% or

% % \re{#1 CP decomposition for multi-dimensional time series data -> most for completion/imputation task}

% \ziyue{comments: distinguish general framework v.s. specific model choice: e.g., tensor decomposition v.s. tensor decomposition, pseudo graph v.s. graph constructed by k-means}

% \textbf{[} Tensor decomposition methods have gained widespread popularity and efficacy in analyzing time series data across diverse disciplines, like neuroscience \cite{cong2015tensor}, transportation \cite{chen2019bayesian} and economics \cite{wang2022high}, due to its capability to exploit the inherent cross-dimensional dependencies and extract concise representations. 
% The CANDECOMP/PARAFAC (CP) tensor decomposition \cite{k:09} emerges as a leading framework which factorizes tensors into a linear combination of low-rank components with weight vectors serving as the extracted features, e.g., a three-dimensional tensor $\mathcal{X}$ is decomposed into three mode matrices along each dimension, $\mathbf{A,B,C}$, with a weight vector $\mathbf{w}$.
% It has been vastly employed for dimensionality reduction \cite{chang2023modelling} and downstream inference tasks such as imputation and prediction \cite{li2020tensor}. 
% % \re{#2 reason: only focus on fitness -> ATD alignment but pair-wise}
% Traditional tensor decomposition models mainly learn the parameters with the supervision of reconstruction error. For instance, \re{as shown in Fig. \ref{fig:motivation}} (a), $\mathbf{w,A,B,C}$ are learned by minimizing the $\| \mathcal{X} - \llbracket  \mathbf{w,A,B,C} \rrbracket \|_2^2$ (with details later). However, this paradigm can only ensure a good restoration from the original tensor but can not guarantee to preserve the hidden class pattern well, \re{due to the nonuniqueness and the rotation invariance of the decomposition results,} e.g., the current transformations may inadvertently distort the features essential for classification.  
% Therefore, limited attention has been directed towards exploring its applicability in the realm of time series classification tasks. \textbf{]}


% \textbf{[}\ziyue{The key point for ATD only using InfoNCE is: we don't know the label, and self-self is the only 100\% correct positive samples.} As the first attempt, ATD incorporates contrastive SSL with tensor decomposition to boost classification power by involving transformation invariance loss \citep{y:22}. However, the instance-wise contrast ignores the inherent class similarity. \textbf{]} \ziyue{This is the most important paragraph, but the shortest.}

% \textbf{[} To address the weakness of instance-wise contrastive learning, various models have been presented to encode the semantic structure of data. For example, prototypical contrastive loss is designed by estimating the centroid of clusters for contrast \cite{li2020prototypical} and covariance contrast objective is discussed to include feature covariance for guidance \cite{zhu2022tico}. Typically, leveraging blocks of positive and negative data can better preserve class information than instance pairs \cite{arora2019theoretical}. Inspired by recent works, We aims to incorporate the class-alignment principle into CP decomposition to improve the discriminative power by emphasizing inter-class variations while minimizing intra-class variations. \textbf{]}

% % \re{propose PCT -> with better positive and negative samplers -> block-wise contrastive learning -> }
% \textbf{[} Since the solution of CP decomposition is not identifiable and rotation-invariant \cite{k:09}, the objective is to find the feature space with maximum class-variability by iteratively estimating class labels and minimizing contrastive losses under reconstruction constraint. 
% Specifically, pseudo graph constructed by k-means clustering \ziyue{here we don't need to specify k-means, but in the implement, we can say we just ``choose'' k-means} is introduced as auxiliary information to guide the graph contrast and augmentation based instance contrast is also included to mitigate class-irrelevant noise.
% It is equivalent to the classical SampledNCE framework \cite{hamilton2017inductive} with a well-designed Laplacian matrix that gives different impact of different contrast sources and also enjoys block-wise contrastive property.
% Then we jointly optimize the contrastive objectives and CP decomposition reconstruction objective using Alternative Least Square (ALS). \textbf{]}

% % \re{contributions: 
% % - pseudo graph guided contrastive learning 
% % - cyclic optimization algorithm with guarantees - search the direction best preserving class information
% % - extensive numerical experiments and visulization for insights <- may present the performance improvement ratio here
% % }

% The main contributions of this work are as follows:

% \begin{itemize}

%     \item We develop a novel Pseudo-graph Contrastive Tensor (PCT) Decomposition approach, enabling CP tensor decomposition for time series classification by introducing both instance-alignment and class-alignment principle for both semantically meaningful and discriminative representations.

%     \item The proposed joint contrastive objective is shown to enjoy block-contrastive loss property which theoretically outperforms instance-wise contrastive losses.

%     \item  An unsupervised alternative optimization algorithm is designed to iteratively estimate the pseudo graph and jointly minimize the contrastive losses and regularized reconstruction loss. We also show that the subproblem for feature vector is exact to optimize the constrained contrastive objective restricted by reconstruction error.

     
% \end{itemize}





